Exploring the Design Space of Deep Convolutional Neural Networks at Large Scale

In recent years, the research community has discovered that deep neural networks (DNNs) and convolutional neural networks (CNNs) can yield higher accuracy than all previous solutions to a broad array of machine learning problems. To our knowledge, there is no single CNN/DNN architecture that solves all problems optimally. Instead, the "right" CNN/DNN architecture varies depending on the application at hand. CNN/DNNs comprise an enormous design space. Quantitatively, we find that a small region of the CNN design space contains 30 billion different CNN architectures. In this dissertation, we develop a methodology that enables systematic exploration of the design space of CNNs. Our methodology is comprised of the following four themes. 1. Judiciously choosing benchmarks and metrics. 2. Rapidly training CNN models. 3. Defining and describing the CNN design space. 4. Exploring the design space of CNN architectures. Taken together, these four themes comprise an effective methodology for discovering the "right" CNN architectures to meet the needs of practical applications.

==> chapters/00_glossary.tex <==
\chapter*{Glossary}
\addcontentsline{toc}{chapter}{Glossary}
I'm the glossary

% inference == scoring == deployment == testing == exercising the model. [with a ref for each.]
% activations == activities [krizhevsky14] == data == feature map.
% weights == parameters == (most of which reside inside of filters)
% arithmetic intensity [cite roofline]
% layer: transformation to data (learned or otherwise)
% architecture: specify ``HW arch" or ``neural arch"
% performance: speak in terms of specific perf metric
% average precision (AP): area under PR curve.
% nodes = servers = GPU workers. (we don't ever use "node" in the sense of a neuron or layer)
% batch; local batch; global batch. [and don't say ``minibatch"]
% OPS, IOPS, FLOPS, ``quantity of computation"
% OPS/s, FLOPS/s, ``computation time"
%    ..,perhaps avoid saying ``computational overhead" ... it could vaguely mean OPS or OPS/s 
% accuracy: a ML algorithm's ability to classify/recognize data correctly
% numerical precision
% ``early'' DNN layer: near the input data
% ``late'' DNN layer: near the output classifier
% peak: highest achievable throughput on a particular piece of computational hardware. this can be determined theoretically (e.g. vector lanes * threads * clock rate) or experimentally (e.g. by the most OPS/sec achieved by any implementation of any algorithm [often dense matrix-matrix multiplication] on the processor)
% line rate: peak throughput of network HW
% transfer learning: using a model trained for one domain (e.g. image classification) and adapting it to a new domain (e.g. object detection)



==> chapters/99_extras.tex <==
\chapter{Extra stuff (to integrate into other chapters or delete)}

%\section{Always cite yourself (Ninja citations)}
%
%More recently, our communication-minimizing convolution~\cite{IandolaConv13} techniques have been adopted in NVIDIA Performance Primitives~\cite{NPP} and possibly cuDNN~\cite{cuDNN}.
%
%HOG~\cite{HOG} is used in the scene segmentation method in~\cite{Hoiem08}, which we leveraged for power line idenfification in~\cite{LinearClutter}.
%
%Applying the roofline model to computer vision~\cite{anderson14}...
%
%NVIDIA GPUs have become more flexible in recent years, with functionality such as 64-bit arithmetic, priority-driven work scheduing~\cite{forrest-nvidia-patent}, and [better libraries?].
%
%While decision trees work well for face recognition [CITE Viola-Jones]~\cite{MethMorph}, tree-based approaches haven't shown broad applicability across hundreds of object classes (unlike deep learning, which does show broad applicability).
%
%Pipeline/spatial parallelism~\cite{fusion11, fusion12}
%
%DNNs are good at a wide range of applications such audio~\cite{ashraf15}, text translation [CITE?]...
%
%DPMs have been used in numerous of applications, ranging from vehicle tracking [CITE] to bird classification~\cite{DPD}.
%
%Image pyramids are a useful strategy in multiresolution object detection -- HOGs and convolutional neural nets can both be computed as pyramids~\cite{DPMareCNN, DenseNet}.

\section{Additional papers to cite}

Accelerating or scaling DNN training: \\
%- SparkNet~\cite{SparkNet} \\
%- Purine~\cite{purine} -- shows 12-GPU scaling numbers. \\
%- If I understand correctly Petuum~\cite{Petuum} is a distributed ML framework from CMU, and Poseidon~\cite{Poseidon} is the application of Pentuum to deep neural network training. The Poseidon paper reports a 4.0x speedup when scaling over 8 GPUs. \\ 
    %there are MANY papers on pentuum: https://petuum.github.io/research.html
%- ``Parameter Server" (CMU)~\cite{ParameterServerCMU}. According to parameterserver.org, the framework only does sparse logistic regression so far, but more algorithms may be supported in the future.\\ %may also add the NIPS Workshop version of the Parameter Server paper. (I'm currently citing the OSDI version.)
%- Minerva~\cite{Minerva}. 4x speedup on 8 CPU-only nodes vs 1 CPU-only node.\\
- SINGA~\cite{SINGA}. (TODO: review the speedups. It looks like multi-node, CPU only?) \\
- DIANNE~\cite{DIANNE}. The ``D" in DIANNE stands for ``distributed." However, this does not appear to be a cluster-scale training system. Rather, The ``distributed" aspect of DIANNE is that it does inference on individual mobile devices instead of on a centralized server. \\
- 8-bit approximation implemented in clusterNet~\cite{dettmers-8bit}. (may also cite the clusterNet git repo.) \\
- (Other reference to ``Caffe on Spark," which we can use to point out that Spark is just being used for job scheduling and data preprocessing?) \\

Asynchronous training: \\
- HOGWild~\cite{HOGWild}, DOGWild~\cite{DOGWild}, BUCKWild~\cite{BUCKWild} \\
- Elastic SGD~\cite{EASGD} \\

High-level DNN frameworks: \\
- Caffe~\cite{jia2014caffe} \\
- TensorFlow~\cite{TensorFlow} \\
- Theano [REF] \\
- Chainer [REF] \\
- MatConvNet [REF] \\
- cuda-convnet (1 and 2) \\
- ccv [REF] \\

Broken versions of what we did: \\
- Theano-MPI~\cite{Theano-MPI} (only showed scaling to 8 GPUs)\\
- Caffe-MPI from GTC 2016~\cite{Caffe-MPI} (only showed scaling up to 16 GPUs) \\


%Accelerating DNN computations: \\
DNN computational kernels: \\
- Neon~\cite{neon-code} and maxDNN~\cite{maxDNN} \\
- Boda~\cite{boda-code} \\
- fbfft~\cite{fbfft} \\
- Comparison of computational efficiency for Neon, Caffe, Torch, etc~\cite{bosch-dnn-comparison} \\


DNN architectures and applications: \\
- updated Azizpour paper~\cite{Azizpour15-updated}. (this is the original~\cite{Azizpour15}.) \\
- After we released the SqueezeNet architecture, we learned about a family of CNN architectures called TinyNet, which were designed by B. Xu~\cite{TinyNet}. The proposed {\em TinyNet-B} model proposed by achieves AlexNet-like accuracy with 7.9MB of uncompressed parameters. We learned about this paper after we released SqueezeNet, which has 1.6x fewer parameters than TinyNet-B. \\
- DPMs applied to (3 apps) \\
- AlexNet paper [or other DNN paper] cited by (3 apps) \\
$~~~$ * AS Vemuri. Inter-Operative Biopsy Site Relocalization in Gastroscopy: Application to Oesophagus, 2016. \\
$~~~$ * Accurate classification of protein subcellular localization from high throughput microscopy images using deep learning \\
$~~~$ * D Filipiak, et al. Quantitative Analysis of Art Market Using Ontologies, Named Entity Recognition and Machine Learning: A Case Study \\
$~~~$ * Towards Automated Melanoma Screening: Proper Computer Vision \& Reliable Results \\
$~~~$ * PV Tran. A Fully Convolutional Neural Network for Cardiac Segmentation in Short-Axis MRI \\
- S. Shankar, et al. Refining Architectures of Deep Convolutional Neural Networks. ariXiv, 2016. \\

Solver approaches: \\
- Hessian-free IBM speech SC2014 [TODO: cite] \\

Related techniques: \\
- dense optical flow -- original~\cite{brox:11} and accelerated~\cite{narayanan:10} \\
- Zeiler and Fergus CNN visualization~\cite{zeilerVisualizeCNN} \\ 
- (Bengio?) DNN book \\
-  Bengio, ``Practical Recommendations for Gradient-Based Training of Deep Architectures" %http://arxiv.org/pdf/1206.5533v2.pdf 
- (Song's content on solvers ... may have to dig up the references myself.)

Computational patterns: \\
- View from Berkeley paper [REF] \\
- other select PALLAS/ParLab/Aspire papers [REF] \\

Magic compilers: \\
- Halide [REF] (Can lead in by saying Caffe unofficially supports Halide layers. Then, say that there are several other frameworks with a similar purpose to Halide.) \\
- SEJITS: \\
$~~~$ * copperhead [REF] \\
$~~~$ * stencil specializer [REF] \\
$~~~$ * hindemith [REF] \\
$~~~$ * Boda (also mentioned under `DNN computational kernels')~\cite{boda-code} \\
- Delite [REF] \\


\section{Material to pillage}

\subsection{Hardware DSE vs DNN DSE. (was originally floating around in ch1)}

%\noindent
%TODO table: \\
%ASIP & DNN
%pipeline depth & depth (\# of layers)
%number of processing units & \# of filters
%\# of vector lanes & dimensions of each filter

\noindent
{\bf Differences between Hardware DSE and DNN DSE.} \\

\noindent
{\bf Hardware (processor) DSE:} 
There are a number of units out of which processors are built.
An adder's job is to add. 
A memory controller's job is to control the memory. 
These and other units can be composed together without changing the behavior of the individual units. 
If an individual unit's behavior change when composed with other units, this is a bug. \\

\noindent 
{\bf DNN DSE:} 
In a DNN, each layer (and indeed each trainable parameter) has no specific pre-defined purpose. 
Changing the dimensionality of layer $L_i$ will certainly change the functions learned in layer $L_{i+1}$.
Even changing the random number generator's seed will change the functions learned by all layers. 
However, we can empirically observe that there are many functions (i.e. many different DNN architectures, and many random seeds for each DNN architecture) that are equally good at solving a particular task such as classifying images, or recognizing speech, or recognizing human actions in videos.
However, unlike the case of DSE in computational hardware where all units have pre-defined functionality, it is an intrinsic property of DNNs that the units of a DNN do {\em not} have predefined functionality (and if they did, there would be no learning in our machine learning).
All that is required is that, at an end-to-end level, the DNN should be trainable to solve a problem such as classifying images with high accuracy; if not, it's a bug.

\subsection{Old intro to Chapter 4}
Deep neural networks comprise an extremely large design space, [which most DNN architects find to be daunting].
While it is true that there are only a handful of commonly-used DNN computational primitives (e.g. convolution, pooling, dropout, etc), there are many ways of arranging these primitives into a deep neural network architecture.
For example, the composition and total number of layers is selected by the DNN architect, and considering that some recent DNN architectures have 1000 layers or more [cite Highway Networks and ResNet], there is an exponentially large number of permutations in which different types of DNN layers can be composed.
Further, within each layer, there are a number of dimensions to be selected by the DNN architect -- e.g. in a convolution layer, the number of filters and spatial resolution of filters are user-selectable.
Also, the initialization of parameters inside of filters (e.g. initialization of parameters to gaussian noise with a per-layer user-selectable standard deviation) comprises a large space of options.
% especially considering that each layer in a DNN can be initialized differently [if the architect wishes to do that].

Despite the large size of the DNN design space, we have identified a number of strategies that make it easier to reason about this design space.
Before we can describe these strategies, we first provide a solid explanation of the key building blocks of DNNs, as well as their dimensional properties in Section~\ref{sec:building-blocks}.
Then, we work a number of numerical examples in Section~\ref{sec:understanding-dimensionality} and Section~\ref{sec:avoid-mistakes}, which should help the reader to build up intuition about the dimensionality of individual DNN layers, as well as how dimensionality from one layer impacts the dimensionality of the following layer.
At this stage, an important fact will become clear: while a huge amounts of computation is necessary to train a DNN and evaluate its accuracy, virtually every other property of a DNN can be resolved either with closed-form calculations, or with minimal microbenchmarks.
For example, we can figure out the number of parameters and the number of arithmetic operations in a DNN architecture with some straightforward closed-form calculations.
Furthermore, we can understand the computational speed (and computational efficiency, and energy efficiency) of a DNN architecture with small microbenchmarks that take less than a minute to run.

The solver approach also has an impact on training time and accuracy; we outline some key aspects of this in Section~\ref{sec:solver-approaches}.

Putting this knowledge to work, we are able to precisely understand the shape of the design space in terms of computational overhead and communication overhead.
Without training any DNNs, we can pinpoint the regions of the DNN architectural space that will train efficiently on a 512 GPUs, or regions that in which models are small enough to fit in on-chip memory, or regions that have a feasible number of arithmetic operations per frame. 
In Section~\ref{sec:playbook}, we will present a playbook in which, for each user-selectable hyperparameter that impacts training time, we show how to modify that hyperparameter to deterministically computational efficiency.
We also impart our intuition on how to select these hyperparameters to improve accuracy, and how to use the hyperparameters to maximize accuracy on a practical (limited) budget of model size or computation.

\subsection{In what situations are DNNs particularly useful?}
DNNs are particularly good at learning a mapping from {\em data} to {\em some analysis of that data}.
Depending on the task at hand, the analysis problem may be defined in a number of ways.
These are a few common problem definitions that DNNs are often well-equipped to address:
\begin{itemize}
	\item 	{\bf Decomposing} data (e.g. segmenting an audio stream into individual words, or segmenting a photo into outlines of individual objects)
	\item	{\bf Classifying} data (e.g. identifying that a text document is written in German, or identifying which videos were recorded outdoors.)
	\item	{\bf Predicting} a future outcome (e.g. TODO. finance? sports video? Ali Farhadi's CVPR on predicting motion?)
	\item	{\bf Reidentifying} data (e.g. identifying copyrighted text, audio or visual content; or tracking a vehicle over multiple security cameras)
	\item	{\bf Synthesizing} more data (e.g. corpus of art $\rightarrow$ more art)
	\item	Selecting and actuating a {\bf motion} (e.g. motion planning for a robot based on sensory inputs)
\end{itemize}



\section{Common DNN usage patterns in computer vision}
TODO figure: [train on imagenet (1-3 weeks)] $\rightarrow$ [fine-tune on target application (1-3 hours)].

[TODO: autonomous driving motivation]
Perhaps use the ``control is pretty well understood; perception is hard part'' argument here... can mention airplanes as a case where autonomous works because perception is less complex even though control is 3D instead of 2D.

Let us consider {\em autonomous driving} as a motivating and illustrative example of how CNNs are applied to computer vision.
[Perhaps mention -- maps tell you where the road is supposed to be ... but not construction, pedestrians, weather, other cars, and other temporary obstacles.]
Identification of obstacles and other road users is a key requirement to make autonomous vehicles safe.

[Explain classification vs detection.]
[Make a picture of ``parking lot" (classification) vs ``individual cars'' (detection)]

PASCAL is one of the most widely used datasets for training and evaluating object detection methods, and PASCAL has approximately 10000 images labeled with a total of (TODO?) bounding boxes~\cite{PASCAL}.
Training a CNN on the PASCAL training set yields a modest [TODO: be specific] accuracy improvement [TODO: ref original R-CNN paper~\cite{R-CNN}] over the previous baseline of Deformable Parts Models (DPMs)~\cite{DPM-journal} [TODO: other DPM refs].
To further improve accuracy with all else held constant, {\em pretraining} a CNN on ImageNet and then continuing training (i.e. finetuning) the CNN on the PASCAL training set further improves accuracy on the PASCAL test set by [20 percentage-points] 

Also discuss further accuracy improvements, in papers such as... \\
- Fast R-CNN~\cite{Fast-R-CNN}, \\
- Faster-R-CNN~\cite{Faster-R-CNN} \\
- (TODO)

A number of reasons for this ``better accuracy with ImageNet pretraining'' phenomenon have been proposed [but let us first understand the stuff that came before CNNs on PASCAL].
In 2012, Zhu \etal performed a suite of experiments to evaluate how the number of training examples affects the accuracy of object detectors~\cite{Zhu12}.
This study was carried out using DPMs and other pre-deep-learning object detection techniques.
To summarize the findings, DPMs have nearly identical accuracy X samples as 10X samples [I need to read this pap more carefully... it discusses 80\% AP on PASCAL in some places, and I am confused].
%[deleted] In DPMs and other pre-deep-learning object recognition techniques, [Vondrick et al] found that adding more training data helped in the range of [1 to 1000 images], and beyond this point a model would saturate and not improve in accuracy when presented with additional labeled data.
%[TODO] However, [TODO: find NIPS 2014 paper in which this was an appendix] shows that CNNs achieve more accuracy with more training data [TODO: stats].

From [2013 to 2016], object detection accuracy on PASCAL has increased from [50 some-odd percent] to [80 some-odd percent].
This improvement has come from the development of better CNN architectures.
These new architectures are deeper [TODO: cite VGG] and are also able to do both classification and localization within a single architecture [TODO: cite faster R-CNN and OverFeat].
For [good safety] in autonomous driving, an important area of further research is to continue to design new CNN architectures that detect objects with even higher accuracy.
If we propose a new CNN architecture, ``NewNet'', let us now consider what is required to train this CNN on the PASCAL dataset and achieve high accuracy.
First, we need to train NewNet to perform image classification ImageNet -- which may take 3 weeks if NewNet has a similar quantity of computation as the GoogLeNet CNN architecture.
Then, we make modest modifications to NewNet to enable object localization as well as object classification [TODO: expand on thee changes].
Finally, we finetune [i.e. resume training] on the PASCAL object detection training set, and this takes roughly 8 hours [if NewNet has similar computational complexity to GoogLeNet].
At this point, we can evaluate the accuracy on the PASCAL test set.
We illustrate this process in Figure [TODO].
%save for later in this chapter: look how much more time is spent on ImageNet training than on PASCAL finetuning.
%TODO: put this in the context of DSE ... we need to do the aforementioned steps for MANY CNN architectures.


\section{CNNs with many channels of input}
TODO: integrate into paragraphs: \\
- Video activity recognition on Sports-1M using LSTMs~\cite{Sports1M-2015} \\
- Human activity recognition on TRECVID, concatenating 7 video frames as input to a CNN~\cite{Ji2010} \\

Karpathy \etal evaluate a number of CNN-based approaches to identifying human actions in videos~\cite{Sports1M}.
One of the approaches is {\em early fusion} of video frames: the authors concatenate groups of 10 video frames in the channel dimension.
Since each frame is a 3-channel RGB image, this forms a 30-channel grid of input to the CNN.


\subsection{Old verison: Changing the height and width of the input data}

\noindent
references to collect: \\
- places2~\cite{places2} \\
- cifar~\cite{CIFAR} \\
% additional papers that resize ImageNet images to 256x256 or similar \\
- Ross's image warping (in supp material)~\cite{R-CNN-supp} \\
%    R-CNN paper (original one): supplementary material
%    https://www.cs.berkeley.edu/~rbg/papers/r-cnn-cvpr-supp.pdf
%    "A pilot set of experiments showed that warping with context padding (p = 16 pixels) outperformed the alternatives by a large margin (3-5 mAP points)."

%info to collect: \\
% height and width (min and max) in ImageNet-1k \\
% height and width (min and max) frame size in VIRAT \\
% range of *object* sizes in VIRAT \\
% summary of image-size experiments in VGG paper \\

On the ImageNet~\cite{imagenet} dataset, the image sizes range from [TODO: MIN] to [TODO: MAX]. 
Many [authors of CNN papers] have simply resized ImageNet training and testing images to a fixed size, such as 256x256 [REF].
However, [VGG authors ... and others?] experimented with various image [(re)sizes] and found that [320xXXX] generates a [X] percentage-point improvement in accuracy compared to [256xXXX].
[TODO: places2 and sports-1m image sizes]
[TODO: CIFAR image sizes]

So far, we have discussed image resolutions for {\em image classification} on datasets such as ImageNet.
However, the ideal image size may depend on the problem at hand.
[Ross: warp vs. pad vs. midway between. REF? Look for a reference. Can fall back on Ross's ICCV 2013 ImageNet talk if necessary.]
[Mention: Faster R-CNN~\cite{Faster-R-CNN} takes a full image as input, and you get to select the resolution.]

For detecting individual objects in large and complex scenes, even higher image resolutions may be beneficial.
For example, the VIRAT~\cite{VIRAT} object detection dataset has hundreds of labeled objects in some frames [TODO: show example frame].
VIRAT was recorded with [high definition ... exact resolution?], but even at this high resolution, some objects are just [SIZE?] pixels wide.
Thus far, we have not seen literature on directly applying approaches such as Faster R-CNN to VIRAT.
But, we expect that achieving high accuracy on VIRAT would require ingesting very high resolution images into Faster R-CNN.

We have established that there are number of scenarios where it is sensible to apply CNNs to higher resolution images.
Let us now apply NiN~\cite{NiN} to 4x larger input images -- that is, we increase the height and width each by a factor of 2, so the number of pixels increases by 4x.


\noindent
TODO: \\
- 224 vs 256 ... random cropping. discuss? \\
- discuss FC layers and resizing? \\

Dealing with ``4.2x vs 4x''... \\
- In terms of output and computation, we land slightly above 4x (due to rounding on downsampling sizes ... TODO: provide details). \\
- could clamp everything to 4x, or \\
- could put precise measurements in $\Delta$ boxes in the chart.

%In terms of computation, this will follow the same principle as Section~\ref{sec:early-downsampling} (i.e. roughly 4x change if the input height and width each change by a factor of 2).
%In terms of number of parameters, this will follow the same principle as Section~\ref{sec:early-downsampling} (i.e. no change).
%In terms of scalability... this is free scale-out if we increase input data height and width.

\section{More trimmings from chapter 2}

\noindent
Notes to put somewhere: \\
- for most CNNs, the quantity of computation is known {\em offline} and does not change dynamically \\ 

	\begin{table*}[h!]
		\footnotesize
		\caption[Metrics for evaluating DNNs.]{Metrics for evaluating DNNs. (``Inf" is short for ``Inference.")}
		\label{T:metrics}
		\centering
		\begin{tabulary}{\linewidth}{|C|C|C|C|C|C|C|C|C|C|C|C|C|C|C|C|} %thx: tex.stackexchange.com/questions/238018
			\hline
			& Accuracy & \multicolumn{2}{c|}{Time} & \multicolumn{2}{c|}{FLOPS} & \multicolumn{2}{c|}{Power} & \multicolumn{2}{c|}{Energy} & \multicolumn{2}{c|}{Cost} & \multicolumn{2}{c|}{Model size}  \\ \hline
			& Inf & Train & Inf & Train & Inf & Train & Inf & Train & Inf & Train & Inf & Train & Inf  \\ \hline
			%		  [none]            & \ck &         &      &          &     &          &      &         &       &         &      &         &        \\ \hline
			[REF Time]      & \ck & \ck    &      &          &     &          &      &         &       &         &      &         &        \\ \hline
			2hr alexnet [REF]& \ck &         & \ck &          &     &          &      &         &       &         &      &         &        \\ \hline
			[MSR CTC]     & \ck &         &       &     ?   & \ck &        &      &         &       &         &      &         &        \\ \hline
			Pratt [REF]       & \ck &         &      &          &     &          &  \ck &       &       &         &      &         &        \\ \hline
			Berg [REF]       & \ck &         &      &          &     &          &      &         &  \ck &        &      &         &        \\ \hline
			Vondrick [REF]& \ck &         &      &          &     &          &      &         &       &         & \ck &         &        \\ \hline
			Han [REF]       & \ck &         &      &          &     &          &      &         &       &         &       &         & \ck    \\ \hline
			%TODO: Anderson, Iandola, and Keutzer
			{\bf Chapter 3}& \ck &  \ck   &      & \td    &      & \td    &      &    \td &       & \td   &       & \ck    &        \\ \hline % Chapter \ref{ch:scale-up} 
			{\bf Chapter 5}& \ck &  \td   & \td &         & \td &         & \td &        &   \td &         &  \td &         &  \td  \\ \hline % Chapter \ref{ch:exploring} 
		\end{tabulary}
	\end{table*}

\section{More trimmings from Chapter 4}
%\section{Hierarchically understanding the CNN design space}
%\label{sec:hierarchically}
%\noindent
%High level abstractions comprised of multiple convolution layers: \\
%- Inception modules \\
%- Resnet modules \\
%- We will present our Fire modules in the next chapter \\


\subsection{TODO: stuff to add}
Most solvers expose the hyperparameters of {\em batch size} and {\em learning rate}.

\noindent
Brief discussion of... \\
- batch size \\
- learning rate {\em schedule} \\
- momentum \\
- weight decay (including ResNet's innovation here) \\
- number of epochs \\


{\bf Batch size.}
(TODO)

{\bf Learning rate}
Our intuition [from empirical research in Chapter 3] is that larger batch sizes go well with larger learning rates.

Difficult to assess {\em how many epochs needed}, given that researchers often use a learning rate schedule that [tracks the epoch index].

\section{Why we're so focused on CNN architectures}
Given a particular problem (e.g. in the domain of text, audio, or vision) and the ability to obtain appropriate labeled data to train models to solve the problem, a CNN architect must carefully consider and explore a number of design choices (DC's) including the following:
\begin{itemize}
	\item {\bf DC1.} The design of the CNN architecture.
	\item {\bf DC2.} The approach for initializing the CNN architecture's model parameters prior to training.
	\item {\bf DC3.} The optimization methodology or {\em solver approach} used to train the model.
\end{itemize}

We now present a few observations on the implications of these design choices, as well as how these design choices have been covered in the literature so far.

CNN architecture (DC1):
\begin{itemize}
	\item The choice of CNN architecture is discussed in relatively little detail in the literature. Out of the thousands of computer vision and CNN papers that have appeared in the last few years, relatively few papers propose a substantially new CNN architecture, much less to propose and evaluate many new CNN architectures.
	\item The choice of CNN architecture directly effects the quantity of computation and the speed that can be achieved during both training and inference. The specific ways in which the CNN architecture impacts the computational footprint is not widely discussed in the literature.
\end{itemize}

Model parameter initialization (DC 2) and Solver approach (DC 3).
\begin{itemize}
	\item Model parameter initialization and solver approaches are widely discussed in the literature. {\em Optimization} is a field with a long history and a wide following, and many optimization experts have recently refocused their careers on optimization methods for neural networks.
	\item The choice how initialize model parameters and the choice of solver approach impacts the number of epochs (i.e. passes through the training set) required to achieve a given level of accuracy.\footnote{Further, DC2 and DC3 can influence the maximum accuracy that can be achieved when training a specific CNN architecture.} Thus, DC2 and DC3 impact the quantity of computation and the time required to {\em train} CNN models. However DC2 and DC  do not impact the quantity of computation or achievable speed during {\em inference}.
\end{itemize}


\section{Solver approaches other than SGD}
Some research has emerged on solver approaches other than SGD for training CNNs.
%Given our orientation toward computational efficiency and scalability, we are particularly [hungry for] solver approaches that expose more parallelism to accelerate training. %that expose more parallelism and/or require fewer iterations.
In Chapter~\ref{ch:scale_up}, we showed competitive results with a batch size of 1024, but at larger batch sizes our experience is that the training process either diverges or converges to a sub-optimal accuracy level.
Recall from Chapter~\ref{ch:scale_up} that, on a fixed number of epochs, doubling the batch size doubles the degree of parallelism (requiring a total of $\frac{1}{2}$ as much total communication during training).
Therefore, an alluring problem is to identify solver approaches that can converge to high accuracy with a reasonable number of epochs and {\em a large batch size}.
A promising direction is the area of {\em second-order optimization}, which consists of [TODO].
[take second derivatives, these derivatives will be `more accurate' and let you `see farther', and you'll need less of them in total.]

A number of recent results have emerged that use second-order optimization.
[though, predictably, each of them has at least one fatal flaw.]

\noindent
papers on second-order CNN training... \\
- O. Vinyals and D. Povey, "Krylov Subspace Descent for Deep Learning," in AISTATS, 2012~\cite{vinyals12}. \\
- Parallel Deep Neural Network Training for Big Data on Blue Gene/Q. ``we explore CNN training using the data parallel Hessian-free 2nd order optimization algorithm."~\cite{ibmSC14} \\
- IBM: ``Optimization Techniques to Improve Training Speed of Deep Neural Networks for Large Speech Tasks." Claim a 3x speedup on English Broadcast News dataset. ~\cite{ibm13} \\


\section{More trimmings from Chapter 5}
	
	Some model compression approaches have greater impact than others on the model's accuracy.
	The Deep Compression and EIE work by Han \etal ... TODO
	Meanwhile, XNOR-Net... TODO

	References to integrate: \\
	- Jaderberg model compression~\cite{jaderberg2014} \\
	- XNOR-net~\cite{XNORnet} (does hurt accuracy) \\
	
	SqueezeNet has also been applied in new research in a number of ways:
	
\begin{itemize}
		\item SqueezeNet neural art~\cite{SqueezeNet-NeuralArt}.
		%https://github.com/pavelgonchar/neural-art-mini
\end{itemize}


%\item William Bokui Shen (CS231 student w/ Song Han) exploring SqueezeNet with bypass connections:
%http://cs231n.stanford.edu/reports2016/410_Report.pdf

%SqueezeNet is prominently featured in this blog post, too: %http://terryum.io/ml_theory/2016/06/05/DeepLearningPapers/ 
% Terry T. Um. "Some trends of deep learning researches." 2016.
%  After quoting the motivation section from the SqueezeNet paper, the author goes on to write, "Now, accuracy is not the only metric which deep learning researchers concerns. Based on better knowledge on the mechanisms of CNN, researchers are trying to reduce the size of CNNs."
%  
% DeepDetect (server-side support for Caffe) -- the DeepDetect code distribution now includes SqueezeNet:
%https://github.com/beniz/deepdetect/tree/master/templates/caffe/squeezenet 


%\section{Recently-appearing related work} 
% Network Trimming: only 2.7x compression.
% http://arxiv.org/pdf/1607.03250v1.pdf
		


